Computation of extreme eigenvalues in higher dimensions using block tensor train format

We consider an approximate computation of several minimal eigenpairs of large Hermitian matrices which come from high--dimensional problems. We use the tensor train format (TT) for vectors and matrices to overcome the curse of dimensionality and make storage and computational cost feasible. Applying a block version of the TT format to several vectors simultaneously, we compute the low--lying eigenstates of a system by minimization of a block Rayleigh quotient performed in an alternating fashion for all dimensions. For several numerical examples, we compare the proposed method with the deflation approach when the low--lying eigenstates are computed one-by-one, and also with the variational algorithms used in quantum physics.

==> tikz/ttdef <==
% Rectangle node with diagonal fill
% Author: Mark Wibrow

\makeatletter

% Shape 'rectangle with diagonal fill'
%
% Inherits everything from rectangle except the behind background path.
%
\pgfdeclareshape{rectangle with diagonal fill}
{
    % This bit from \pgflibarayshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
   \inheritanchor[from=rectangle]{north}
   \inheritanchor[from=rectangle]{north west}
   \inheritanchor[from=rectangle]{north east}
   \inheritanchor[from=rectangle]{center}
   \inheritanchor[from=rectangle]{west}
   \inheritanchor[from=rectangle]{east}
   \inheritanchor[from=rectangle]{mid}
   \inheritanchor[from=rectangle]{mid west}
   \inheritanchor[from=rectangle]{mid east}
   \inheritanchor[from=rectangle]{base}
   \inheritanchor[from=rectangle]{base west}
   \inheritanchor[from=rectangle]{base east}
   \inheritanchor[from=rectangle]{south}
   \inheritanchor[from=rectangle]{south west}
   \inheritanchor[from=rectangle]{south east}

   \inheritbackgroundpath[from=rectangle]
   \inheritbeforebackgroundpath[from=rectangle]
   \inheritbehindforegroundpath[from=rectangle]
   \inheritforegroundpath[from=rectangle]
   \inheritbeforeforegroundpath[from=rectangle]

  % Now do the background filling.
   \behindbackgroundpath{%
       % \southwest and \northeast defined by rectangle, but
       % (somewhat annoyingly) not \southeast and \northwest
       % so use this workaround.
       \pgfextractx{\pgf@xa}{\southwest}%
       \pgfextracty{\pgf@ya}{\southwest}%
       \pgfextractx{\pgf@xb}{\northeast}%
       \pgfextracty{\pgf@yb}{\northeast}%
       \ifpgf@diagonal@lefttoright
           \def\pgf@diagonal@point@a{\pgfpoint{\pgf@xa}{\pgf@yb}}%
           \def\pgf@diagonal@point@b{\pgfpoint{\pgf@xb}{\pgf@ya}}%
       \else
           \def\pgf@diagonal@point@a{\southwest}%
           \def\pgf@diagonal@point@b{\northeast}%
       \fi
       \pgfpathmoveto{\pgf@diagonal@point@a}%
       \pgfpathlineto{\northeast}%
       \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
       \pgfpathclose
       \ifpgf@diagonal@lefttoright
           \color{\pgf@diagonal@top@color}%
       \else
           \color{\pgf@diagonal@bottom@color}%
       \fi
       \pgfusepath{fill}%
       \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
       \pgfpathlineto{\southwest}%
       \pgfpathlineto{\pgf@diagonal@point@b}%
       \pgfpathclose
       \ifpgf@diagonal@lefttoright
           \color{\pgf@diagonal@bottom@color}%
       \else
           \color{\pgf@diagonal@top@color}%
       \fi
       \pgfusepath{fill}%
   }
}

\newif\ifpgf@diagonal@lefttoright
\def\pgf@diagonal@top@color{white}
\def\pgf@diagonal@bottom@color{gray!30}

% Use these with PGF
\def\pgfsetdiagonaltopcolor#1{\def\pgf@diagonal@top@color{#1}}%
\def\pgfsetdiagonalbottomcolor#1{\def\pgf@diagonal@bottom@color{#1}}%
\def\pgfsetdiagonallefttoright{\pgf@diagonal@lefttorighttrue}%
\def\pgfsetdiagonalrighttoleft{\pgf@diagonal@lefttorightfalse}%

% Use these with TikZ
\tikzoption{diagonal top color}{\pgfsetdiagonaltopcolor{#1}}
\tikzoption{diagonal bottom color}{\pgfsetdiagonalbottomcolor{#1}}
\tikzoption{diagonal from left to right}[]{\pgfsetdiagonallefttoright}
\tikzoption{diagonal from right to left}[]{\pgfsetdiagonalrighttoleft}
\makeatother
%
% Local definitions
%
\tikzstyle{core}=[rectangle,draw=black,fill=white,thick,minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corel}=[rectangle with diagonal fill, diagonal from left to right, diagonal top color=black!05, diagonal bottom color=white, draw=black, thick,minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corer}=[rectangle with diagonal fill, diagonal from right to left, diagonal top color=black!05, diagonal bottom color=white, draw=black, thick,minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corell}=[rectangle,thick,draw=black,pattern=north west lines,pattern color=black!60, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corerr}=[rectangle,thick,draw=black,pattern=north east lines,pattern color=black!60, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corez}=[rectangle,thick,draw=black,fill=black!10, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corex}=[rectangle,thick,draw=black,fill=black!25, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corev}=[rectangle,thick,draw=white,fill=white, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{bond}=[draw]
\tikzstyle{void}=[circle,minimum size=\TIKZlspan]
\endinput

